Implementing a synthetic magnetic vector potential in a 2D superconducting qubit array

Superconducting quantum processors are a compelling platform for analog quantum simulation due to the precision control, fast operation, and site-resolved readout inherent to the hardware. Arrays of coupled superconducting qubits natively emulate the dynamics of interacting particles according to the Bose-Hubbard model. However, many interesting condensed-matter phenomena emerge only in the presence of electromagnetic fields. Here, we emulate the dynamics of charged particles in an electromagnetic field using a superconducting quantum simulator. We realize a broadly adjustable synthetic magnetic vector potential by applying continuous modulation tones to all qubits. We verify that the synthetic vector potential obeys requisite properties of electromagnetism: a spatially-varying vector potential breaks time-reversal symmetry and generates a gauge-invariant synthetic magnetic field, and a temporally-varying vector potential produces a synthetic electric field. We demonstrate that the Hall effect--the transverse deflection of a charged particle propagating in an electromagnetic field--exists in the presence of the synthetic electromagnetic field.

==> ACPreamble.tex <==
\usepackage{graphicx}
\usepackage{dcolumn}
\usepackage{bm}
\usepackage{bbm}
\usepackage{multirow}

\usepackage{cancel}
\usepackage[normalem]{ulem}

\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{amsfonts}
% \usepackage{amsbsy} 
%\usepackage{amscd}

\usepackage{braket}
\newcommand{\ketbra}[2]{\ket{#1}\!\!\bra{#2}}
\newcommand{\Ketbra}[2]{\Ket{#1}\!\!\Bra{#2}}

\usepackage[all,matrix,cmtip]{xy}
\usepackage{mathtools}

%\usepackage{csquotes}
%\MakeOuterQuote{"}

\usepackage{color}
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{dblue}{rgb}{0,0,0.4}
\definecolor{green}{rgb}{0,1,0}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\definecolor{pastelblue}{RGB}{20,93,160}

\definecolor{brn}{rgb}{.8,.4,.0}
\definecolor{redo}{rgb}{1,.5,.0}
\definecolor{ddgrn}{rgb}{0,0.4,0}
\definecolor{dgrn}{rgb}{0,0.55,0}
\definecolor{dbl}{rgb}{0,0,0.5}

%\usepackage[colorlinks,citecolor=blue,linkcolor=blue,urlcolor=blue]{hyperref}
% \usepackage[colorlinks,citecolor=pastelblue,linkcolor=pastelblue,urlcolor=pastelblue, pagebackref]{hyperref}
% \hypersetup{
% 	colorlinks,
% 	citecolor=pastelblue,
% 	linkcolor=pastelblue,
% 	urlcolor=pastelblue
% }

\newcommand{\white}[1]{\color{white}{#1}}
\newcommand{\red}[1]{\color{red}{#1}}
\newcommand{\blue}[1]{\color{blue}{#1}}
\newcommand{\green}[1]{\color{green}{#1}}
\newcommand{\dgrn}[1]{\color{dgrn}{#1}}
\newcommand{\dblue}[1]{\color{dblue}{#1}}

\newcommand{\one}{\mathbf{1}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\G}{\mathbb{G}}

\newcommand{\ft}{\leftthreetimes}
\newcommand{\gext}{\leftthreetimes}

\renewcommand{\v}[1]{\boldsymbol{#1}} 
\renewcommand{\t}[1]{\widetilde{#1}} 
\newcommand{\ii}{\hspace{1pt}\mathrm{i}\hspace{1pt}}
\newcommand{\ee}{\hspace{1pt}\mathrm{e}}
\newcommand{\dd}{\hspace{1pt}\mathrm{d}}
\newcommand{\<}{\langle} 
\renewcommand{\>}{\rangle} 
\renewcommand{\=}{\coloneqq}

% \usepackage[superscript,biblabel]{cite}
\newcommand{\Rf}[1]{Ref.~\citen{#1}}
\newcommand{\Rfs}[1]{Refs.~\citen{#1}}
\newcommand{\Eq}[1]{(\ref{#1})} 
\newcommand{\eq}[1]{(\ref{#1})} 
\newcommand{\eqn}[1]{eqn.~(\ref{#1})} 
\newcommand{\Eqn}[1]{Eqn.~(\ref{#1})} 
\newcommand{\scn}[1]{Sec.~\ref{#1}} 

\newcommand{\Tr}{{\rm Tr}} 
\newcommand{\Det}{{\rm Det}} 
\renewcommand{\Im}{{\rm Im}} 
\renewcommand{\Re}{{\rm Re}} 
\newcommand{\ch}{{\rm ch}} 
\newcommand{\sh}{{\rm sh}} 
\newcommand{\prt}{\partial} 
\newcommand{\pt}{\partial} 
\newcommand{\sgn}{{\rm sgn}} 
\newcommand{\up}{\uparrow} 
\newcommand{\down}{\downarrow} 

\newcommand{\ie}{{\it i.e.~}} 
\newcommand{\eg}{{\it e.g.~}} 
\newcommand{\etc}{{\it etc.~}} 
\newcommand{\etal}{{\it et al.~}} 

\newcommand{\bpm}{\begin{pmatrix}}
	\newcommand{\epm}{\end{pmatrix}}
\newcommand{\bmm}{\begin{matrix}}
	\newcommand{\emm}{\end{matrix}}
\newcommand{\bvm}{\begin{vmatrix}}
	\newcommand{\evm}{\end{vmatrix}}



\newcommand{\cA}{ {\cal A} } 
	\newcommand{\cB}{ {\cal B} }
	\newcommand{\cC}{ {\cal C} } 
	\newcommand{\cD}{ {\cal D} } 
	\newcommand{\cE}{ {\cal E} } 
	\newcommand{\cF}{ {\cal F} } 
	\newcommand{\cG}{ {\cal G} } 
	\newcommand{\cH}{ {\cal H} } 
	\newcommand{\cK}{ {\cal K} } 
	\newcommand{\cL}{ {\cal L} } 
	\newcommand{\cM}{ {\cal M} } 
	\newcommand{\cN}{ {\cal N} } 
	\newcommand{\cP}{ {\cal P} } 
	\newcommand{\cR}{ {\cal R} } 
	\newcommand{\cS}{ {\cal S} } 
	\newcommand{\cT}{ {\cal T} } 
	\newcommand{\cO}{ {\cal O} } 
	\newcommand{\cV}{ {\cal V} } 
	\newcommand{\cX}{ {\cal X} } 
	\newcommand{\cY}{ {\cal Y} } 
	\newcommand{\cZ}{ {\cal Z} } 

\usepackage{euscript}
\newcommand\eA           {\EuScript{A}}
	\newcommand\eB           {\EuScript{B}}
	\newcommand\eC           {\EuScript{C}}
	\newcommand\eD           {\EuScript{D}}
	\newcommand\eE          {\EuScript{E}}
	\newcommand\eF          {\EuScript{F}}
	\newcommand\eG         {\EuScript{G}}
	\newcommand\eH         {\EuScript{H}}
	\newcommand\eI           {\EuScript{I}}
	\newcommand\eK         {\EuScript{K}}
	\newcommand\eL          {\EuScript{L}}
	\newcommand\eM          {\EuScript{M}}
	\newcommand\eN         {\EuScript{N}}
	\newcommand\eO         {\EuScript{O}}
	\newcommand\eP         {\EuScript{P}}
	\newcommand\eQ         {\EuScript{Q}}
	\newcommand\eR         {\EuScript{R}}
	\newcommand\eS         {\EuScript{S}}
	\newcommand\eT         {\EuScript{T}}
	\newcommand\eV        {\EuScript{V}}
	\newcommand\eW        {\EuScript{W}}
	\newcommand\eX         {\EuScript{X}}
	\newcommand\eY         {\EuScript{Y}}
	\newcommand\eZ         {\EuScript{Z}}


\newcommand\sA           {\mathsf{A}}
	\newcommand\sB           {\mathsf{B}}
	\newcommand\sC           {\mathsf{C}}
	\newcommand\sD           {\mathsf{D}}
	\newcommand\sE          {\mathsf{E}}
	\newcommand\sF          {\mathsf{F}}
	\newcommand\sG         {\mathsf{G}}
	\newcommand\sH         {\mathsf{H}}
	\newcommand\sI           {\mathsf{I}}
	\newcommand\sJ           {\mathsf{J}}
	\newcommand\sK         {\mathsf{K}}
	\newcommand\sL          {\mathsf{L}}
	\newcommand\sM          {\mathsf{M}}
	\newcommand\sN         {\mathsf{N}}
	\newcommand\sO         {\mathsf{O}}
	\newcommand\sP         {\mathsf{P}}
	\newcommand\sQ         {\mathsf{Q}}
	\newcommand\sR         {\mathsf{R}}
	\newcommand\sS         {\mathsf{S}}
	\newcommand\sT         {\mathsf{T}}
	\newcommand\sV        {\mathsf{V}}
	\newcommand\sW        {\mathsf{W}}
	\newcommand\sX         {\mathsf{X}}
	\newcommand\sY         {\mathsf{Y}}
	\newcommand\sZ         {\mathsf{Z}}

%\usepackage{dsfont}
%\usepackage{eufrak}

%\newcommand{\prop}{\propto} 

\newcommand{\al}{\alpha} 
	\newcommand{\bt}{\beta} 
	\newcommand{\del}{\delta} 
	\newcommand{\Del}{\Delta} 
	\newcommand{\eps}{\epsilon} 
	\newcommand{\veps}{\varepsilon} 
	\newcommand{\ga}{\gamma} 
	\newcommand{\Ga}{\Gamma} 
	\newcommand{\ka}{\kappa} 
	\newcommand{\la}{\lambda} 
	\newcommand{\La}{\Lambda} 
	\newcommand{\om}{\omega} 
	\newcommand{\Om}{\Omega} 
	\renewcommand{\th}{\theta} 
	\newcommand{\Th}{\Theta} 
	% \newcommand{\si}{\sigma} 
	\newcommand{\Si}{\Sigma} 
	\newcommand{\vphi}{\varphi} 

\newcommand{\frmbox}[1]{\begin{center}\fbox{\parbox{3.3in}{\parindent=0pt #1}}\end{center}}

\newcommand{\AC}[1]{{\emph{\dblue{[AC: #1]}} }}

% double angle brakets
\makeatletter
\newsavebox{\@brx}
\newcommand{\llangle}[1][]{\savebox{\@brx}{\(\m@th{#1\langle}\)}%
	\mathopen{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\newcommand{\rrangle}[1][]{\savebox{\@brx}{\(\m@th{#1\rangle}\)}%
	\mathclose{\copy\@brx\kern-0.5\wd\@brx\usebox{\@brx}}}
\makeatother

\newcommand{\cRep}{\cR \mathrm{ep}}
\newcommand{\cVec}{\cV \mathrm{ec}}

\newcommand{\OMA}[1]{({\color{blue}{Omer: #1}})}

\theoremstyle{definition}
\newtheorem{defn}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{thm}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{conj}{Conjecture}
\newtheorem{examp}{Example}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}

\numberwithin{equation}{section}
